An extension of Batanin's approach to globular algebras

In earlier work, Batanin has shown that an important class of definitions of higher categories could be apprehended together simply as monads over globular sets. This allowed him to generalize the notion of polygraph, initially introduced by Street and Burroni for strict categories, to all algebraic globular higher categories. In this work, we refine this perspective and introduce new constructions and properties for this class of higher categories. In particular, we define the notion of cellular extension and its associated free construction, from which we obtain another definition of polygraphs and the adjunction between globular algebras and polygraphs. We moreover introduce two criteria allowing one to use most of the constructions of this article without having to describe explicitly the underlying globular monad.

==> Makefile <==
ARXIV_OUT=arxiv_temp
ARXIV_REMOVED=article.tex temp.tex cimetiere.tex atelier.tex work.tex
PDFLATEX=pdflatex

all: article plain
	# rubber -d -W refs -W misc article

release-plain:
	$(PDFLATEX) '\let\ifdebugmode\iffalse\input{article-plain}'
	biber article-plain
	$(PDFLATEX) '\let\ifdebugmode\iffalse\input{article-plain}'
	$(PDFLATEX) '\let\ifdebugmode\iffalse\input{article-plain}'
	cp article-plain.pdf article-release.pdf

article: satex
	-bibtex article.aux
	pdflatex article.tex

bidule: SHELL:=/bin/bash
bidule:
	sed --debug $$'/iii/{z;rarxiv.tex\n}' test.sty

plain: satex
	rubber -d article-plain

arxiv:
# to be executed in the archive generated by arxiv_archive in order to get the arxiv version
	rubber -d article-plain
	cp article-plain.pdf ../article-arxiv.pdf
	echo "SF: pour mettre à jour le pdf sur le site, faire 'make update_site'."

arxiv_archive: SHELL:=/bin/bash
arxiv_archive:
	rm -rf ${ARXIV_OUT}
	mkdir ${ARXIV_OUT}
	git archive --format=tar HEAD . | (cd ${ARXIV_OUT}; tar xf -)
	rm -r ${ARXIV_OUT}/satex
	make -j4 -C satex satix
	cp -r -L satex ${ARXIV_OUT}/satex
	(cd ${ARXIV_OUT}/satex; rm *.pdf)
	(cd ${ARXIV_OUT};\
	rm ${ARXIV_REMOVED};\
	sed -i 's/\\bibliography{papers}/\\bibliography{article-plain}/' plan.tex;\
	mv papers.bib article-plain.bib;\
	cp ../article-plain.bbl article-plain.bbl;\
	sed -i 's/\\addbibresource{papers.bib}/\\addbibresource{article-plain.bib}/' macros.sty;\
	sed -i $$'/%%% ARXIV-PLACEHOLDER/{z;rarxiv.tex\n}' macros.sty;\
	tar cvzf arxiv.tar.gz *;\
	cp -i arxiv.tar.gz ../arxiv.tar.gz)

#update_site:
#	cp article-arxiv.pdf ~/ens/site-web/articles/forest-rewriting-2021.pdf

satex:
	@make -C ../satex

clean:
	rm -f *.aux *.bbl *.blg *.log *.out *.toc

# article-temp: pdf temporaire pour avoir sur le site le temps que l'on sorte
# l'article officiel
article-temp:
	rubber -d -W refs -W misc article-temp
	cp -u article-temp.pdf article-temp-out.pdf

#article-temp-copy:
#	cp -u article-temp-out.pdf /home/simon/ens/site-web/articles/forest-coherence-2020.pdf

ci:
	git commit . -m "Worked on the article."
	git push

#upload: plain
#	scp article-plain.pdf lix:.webdir/docs/mimram_gray_rewr.pdf

.PHONY: satex


==> arxiv.tex <==
% to be added in the arxiv version (no other pdf allowed, figs must be recomputed)
\usepackage{xkeyval}
\makeatletter
\define@key{satex}{scale}{\def\satex@scale{#1}}
\newcommand{\defsatexfig}[2]{\expandafter\newcommand\csname satexfigure#1\endcsname{#2}}
\renewcommand{\satex}[2][]{%
  \expandafter\let\csname satexfigure0\endcsname\undefined
  \def\satex@scale{0.9}\setkeys{satex}{#1}%
  \IfFileExists{satex/#2.satix}{\input{satex/#2.satix}}{\@latex@error{No
      file #2.satix}.}%
  \vcenter{%
    \hbox{\scalebox{\satex@scale}{%
        \csname satexfigure0\endcsname
      }}}}
\renewcommand{\satexnoscale}{\satex}
\makeatother

==> contenu.tex <==

% Contenu à remettre à un endroit ou explicitement enlever

In order to study functors of the form~$\mcal D \to \mcal C^T$, it is useful to
introduce an abstract characterization for such functors, which is a
specialization in~$\CAT$ of the general description of Eilenberg-Moore objects
given by Street in his formal theory of monads~\cite{street1972formal}. To give
some intuition, note that $T$\algebra can be equivalently described as a
functor~$F \co \termcat \to \mcal C$ together with a natural transformation~$\alpha \co TF \To F$ such that
\[
  \alpha \circ (\eta F) = \unit F
  \qtand
  \alpha \circ (\mu F) = \alpha \circ (T \alpha)
\]
This correspondence extends to more general functors to~$\mcal C^T$ in the form
of the following property, that can be derived from~\cite[Theorem~1]{street1972formal}:
\begin{theo}
  \label{thm:charact-functors-to-EM-cat}
  Given a category~$\mcal D$, the operation which maps a functor~$G \co \mcal D
  \to \mcal C^T$ to the pairs~$(\bigfun U^TG, \bigfun U^T \eps^T G)$ induces a natural
  bijective correspondence between the functors~$\mcal D \to \mcal C^T$ and the
  pairs~$(F,\alpha)$ where~$F \co \mcal D \to \mcal C$ is a functor and~$\alpha
  \co TF \To F$ is a natural transformation such that
\[
  \alpha \circ (\eta F) = \unit F
  \qtand
  \alpha \circ (\mu F) = \alpha \circ (T \alpha)\zbox.
\]
\end{theo}
\noindent In fact, the correspondence of~\cite[Theorem~1]{street1972formal}
relies on a $2$\nbd-adjunction, so that it extends to natural transformations as
well:
\begin{theo}
  Given a category~$\mcal D$ and functors~$G,G' \co \mcal D \to \mcal C^T$, the
  operation which maps a natural transformation~$\beta \co G \To G'$ to~$\bigfun U^T \beta$ induces a bijective correspondence between the natural
  transformation~$G \To G'$ and the natural transformations~$\bar\beta \co \bigfun U^T G \To \bigfun U^T G'$ such that
  \[
    \beta \circ (\bigfun U^T \eps^T G) = (\bigfun U^T \eps^T G')\circ (T \beta)
  \]
\end{theo}

\paragraph{Monadicity}

Let~$(T,\eta,\mu)$ be a monad on a category~$\mcal C$. Given a category~$\mcal
D$ and an adjunction~$\bigfun F \dashv \bigfun U \co \mcal D \to \mcal C$ such that
the monad induced by this adjunction is exactly~$(T,\eta,\mu)$, recall that
there is a canonical functor~$\bigfun H \co \mcal D \to \mcal C^T$, called
\index{comparison functor}\emph{comparison functor}, derived from this
adjunction (\cf~\cite[Theorem~VI.3.1]{mac2013categories}). This functor can also
be defined in the setting of Street using \Cref{thm:charact-functors-to-EM-cat}:
\begin{theo}[{\cite[Theorem~3]{street1972formal}}]
  \label{prop:comparison-functor}
  There is a unique functor~$\bigfun H \co \mcal D \to \mcal C^T$ such that
  \[
    \bigfun U^T \bigfun H = \bigfun U
    \qtand
    \bigfun U^T \eps^T \bigfun H = \bigfun U \eps
  \]
  where~$\eps$ is the counit of~$\bigfun F \dashv \bigfun U$. The functor~$\bigfun H$
  moreover satisfies that~$\bigfun F^T = \bigfun H \bigfun F$ and~$\eps^T \bigfun H = \bigfun H \eps$.
\end{theo}

\noindent A functor~$\mcal {\bar U}\co \mcal {\bar D} \to \mcal {\bar C}$ is
said \index{monadic functor}\emph{monadic} when it has a right adjoint~$\mcal {\bar F} \co \mcal {\bar
  C} \to \mcal {\bar D}$ such that the comparison functor~$\bar{\bigfun H} \co \mcal {\bar D}
\to \mcal {\bar C}^{\bar T}$ is an equivalence of categories, where~$(\bar
T,\bar \eta,\bar \mu)$ is the monad induced by the adjunction~$\mcal {\bar F}
\dashv \mcal {\bar U}$. Monadic functors can be characterized by Beck's
monadicity theorem that we introduce later (\cf \Cref{thm:monadicity}).

==> strcat-precat.tex <==

In this section, we justify the definition of precategories as ``strict
categories without the exchange law'' and recall from~\cite{makkai2005word} how
strict categories can be expressed as precategories satisfying a condition
analogous to the exchange law. This equivalent definition will be used in
particular in the next chapter\link to give an effective description of the free
extension on an $n$\cellular extension, ultimately leading to an efficient
algorithm which solves the word problem on polygraphs of strict categories.

\paragraph{Categories as precategories}
\parlabel{text:strcats-to-precats}

For~$n \in \Ninf$ and~$C \in \nPCat n$, we write~\ref{cond:pcat-to-strict} for the
following property on~$C$:
\begin{enumerateaxioms}[label=(E),ref=(E)]
%\begin{enumerate}[label=(P),ref=(P)]
\item\label{cond:pcat-to-strict} for~$i,k,l \in \N_n$ with~$1 \le i =
  \min(k,l)-1$,~$u \in C_k$ and~$v \in C_l$, if~$u,v$ are $(i{-}1)$\composable,
  then
  \[
    (u \pcomp_{i-1} \csrc_{i}(v)) \pcomp_{i} (\ctgt_{i}(u) \pcomp_{i-1} v) =
    (\csrc_{i}(u) \pcomp_{i-1} v) \pcomp_{i} (u \pcomp_{i-1} \ctgt_{i}(v))\zbox.
  \]
%\end{enumerate}
\end{enumerateaxioms}
Let~$\smash{\nPCatstr n}$\glossary(PCatE){$\nPCatstr n$}{the category of
  precategories which satisfy the exchange condition~\ref{cond:pcat-to-strict}}
be the full subcategory of~$\nPCat n$ of those $n$\precategories~$C$ that
satisfy~\ref{cond:pcat-to-strict}. The condition~\ref{cond:pcat-to-strict} can
be thought as an equivalent for precategories of the exchange law~\ref{cat:xch}
of strict categories. We now introduce a functor from strict $n$\categories to
$n$\precategories which satisfy~\ref{cond:pcat-to-strict} with the following
proposition:
\begin{prop}
  \label{prop:cat-to-precat}
  Given~$n \in \Ninf$, there is a canonical functor~$\Theta^n \co \nCat n \to
  \smash{\nPCatstr n}$.
\end{prop}
\begin{proof}
  Given~$C \in \nCat n$, we define a structure of $n$\precategory on the
  underlying $n$\globular set of~$C$. We keep the identities given by the strict
  $n$\category structure and define the composition operations~$\pcomp_{(-)}$
  on~$C$ based on the composition operations~$\comp_{(-)}$. Given~$i,k,l \in
  \N_n$ with~$i = \min(k,l) - 1$,~$u \in C_k$ and~$v\in C_l$ such that~$u,v$ are
  $i$\composable, we put
  \[
    u\pcomp_iv =
    \unitp{m}{u}\comp_i\unitp{m}{v}
  \]
  where~$m = \max(k,l)$. Axioms~\ref{precat:src-tgt-unit},
  \ref{precat:csrc-tgt}, \ref{precat:compat-id-comp}, \ref{precat:assoc} are
  then direct consequences of the axioms of strict $n$\categories. We only prove
  the first part of~\ref{precat:distrib} since the other is symmetrical.
  Let~$i,j,k,l,l' \in \N_n$ with~$i = \min(k,\max(l,l')) - 1$,~$j = \min(l,l') -
  1$ and~$i < j$,~$u\in C_{k}$, and~$v\in C_{l},v'\in C_{l'}$ such that~$u,v$
  are $i$\composable and~$v,v'$ are $j$\composable. Writing~$m$
  for~$\max(l,l')$, we have
  \begin{align*}
    u\pcomp_i(v\pcomp_j v')
    &=
      \unitp{m}{u}\comp_i\unitp{m}{}(\unitp m v \comp_j \unitp m {v'})
    & \text{(by
      definition of~$\pcomp_{(-)}$)}\\
    &= \unitp{m}{u}\comp_i(\unitp m v \comp_j
      \unitp m {v'})\\
    &= (\unitp{m}{u}\comp_j\unitp{m}{u})\comp_i(\unitp m v \comp_j
      \unitp m {v'})
    & \text{(by \Axr{cat:unital})}\\
    &= (\unitp{m}{u}\comp_i\unitp m
      v)\comp_j(\unitp{m}{u} \comp_i \unitp m {v'})
    & \text{(by \Axr{cat:xch})}\\
    &=
      \unitp{m}{}(\unitp{j+1}{u}\comp_iv)\comp_j\unitp{m}{}(\unitp{j'+1}{u} \comp_i
      v')
    &\text{(by \Axr{cat:id-xch})}\\
    &= (u\pcomp_iv)\pcomp_j(u\pcomp_iv')
    &\text{(by definition of~$\pcomp_{(-)}$)}
  \end{align*}
  which concludes the proof of~\ref{precat:distrib}. Thus,~$C$ is an
  $n$\precategory. We now show that it satisfies the
  condition~\ref{cond:pcat-to-strict} above. So let~$i,k,l \in \N_n$ with~$1 \le
  i = \min(k,l)-1$,~$u \in C_k$ and~$v \in C_l$ such that~$u,v$ are
  $(i{-}1)$\composable. Writing~$m$ for~$\max(k,l)$, we have
  \begin{align*}
    (u \pcomp_{i-1} \csrc_{i}(v)) \pcomp_{i} (\ctgt_{i}(u)
    \pcomp_{i-1} v) &= \unitp{m}{}(u\comp_{i-1}\unitp{k}{\csrc_{i}(v)}) \comp_i
                      \unitp{m}{}(\unitp{l}{\ctgt_{i}(u)} \comp_{i-1} v) & \text{(by definition
                                                                           of~$\pcomp_{(-)}$)}\\
                    &= (\unitp{m}{u}\comp_{i-1}\unitp{m}{\csrc_{i}(v)})
                      \comp_i (\unitp{m}{\ctgt_{i}(u)} \comp_{i-1} \unitp{m}{v}) & \text{(by
                                                                                   \Axr{cat:id-xch})} \\
                    &= (\unitp{m}{u}\comp_{i}\unitp{m}{\ctgt_{i}(u)})
                      \comp_{i-1} (\unitp{m}{\csrc_{i}(v)} \comp_{i} \unitp{m}{v}) & \text{(by
                                                                                     \Axr{cat:xch})}\\
                    &= \unitp{m}{u}\comp_{i-1}\unitp{m}{v} & \text{(by
                                                             \Axr{cat:unital})}\\
                    &= (\unitp{m}{\csrc_{i}(u)}\comp_{i}\unitp{m}{u})
                      \comp_{i-1} (\unitp{m}{v} \comp_{i} \unitp{m}{\ctgt_{i}(v)}) & \text{(by
                                                                                     \Axr{cat:unital})}\\
                    &= (\unitp{m}{\csrc_{i}(u)}\comp_{i-1}\unitp{m}{v})
                      \comp_{i} (\unitp{m}{u} \comp_{i-1} \unitp{m}{\ctgt_{i}(v)}) & \text{(by
                                                                                     \Axr{cat:xch})}\\
                    &= \unitp{m}{}(\unitp{l}{\csrc_{i}(u)} \comp_{i-1} v) \comp_i
                      \unitp{m}{}(u\comp_{i-1}\unitp{k}{\ctgt_{i}(v)}) & \text{(by
                                                                         \Axr{cat:id-xch})}\\ &= (\csrc_{i}(u) \pcomp_{i-1} v) \pcomp_{i} (u \pcomp_{i-1}
                                                                                                \ctgt_{i}(v)) & \text{(by definition of~$\pcomp_{(-)}$)}
  \end{align*} which concludes the proof of~\ref{cond:pcat-to-strict}.

  Thus, for~$n \in \Ninf$, we have defined a mapping~$\Theta^n$ between the
  objects of~$\nCat n$ and the objects of~$\nPCatstr n$. We show that~$\Theta^n$
  extends to a functor~$\Theta^n\co \nCat n \to \nPCatstr n$. Given an
  $n$\functor~$F\co C \to C'$ between two strict $n$\categories~$C$ and~$C'$, it
  is sufficient to show that~$F$ is compatible with the composition
  operations~$\pcomp_{(-)}$. But this is a direct consequence of the definition
  of~$u \pcomp_i v$ as~$\unitp m u \comp_i \unitp m v$ for~$i,k,l,m \in \N_n$
  with~$i = \min(k,l) - 1$ and~$m = \max(k,l)$, and~$u \in C_k,v \in C_l$
  with~$u,v$ $i$\composable, since~$F$ is compatible with~$\unitp m {}$
  and~$\comp_i$.
\end{proof}

\paragraph{Precategories as categories} 

In this section, we prove the converse property, \ie that precategories
satisfying~\ref{cond:pcat-to-strict} are canonically strict categories. For this
purpose, we introduce a functor from~$\smash{\nPCatstr n}$ to~$\nCat n$ with the
following property:
\begin{prop}
  \label{prop:precat-to-cat}
  Given~$n \in \Ninf$, there is a canonical functor~$\bar\Theta^n \co
  \smash{\nPCatstr n} \to \nCat n$.
\end{prop}
\begin{proof}
  Given~$C \in \smash{\nPCatstr n}$, we define a structure of strict
  $n$\category on the underlying $n$\globular set of~$C$. We keep the identities
  given by the structure of $n$\precategory of~$C$ and define the multiple
  composition operations~$\comp_{(-)}$ based on the precategorical composition
  operations~$\pcomp_{(-)}$. For~$i,k \in \N_{n}$ with~${i < k}$, we
  define~$u\comp_iv$ for $i$\composable~$u,v\in C_{k}$ by induction on~$k - i$.
  In the cases where~$i > 0$, we moreover prove that
  \begin{equation}
    \label{eq:parametrized-exch}
    (\tilde u\pcomp_{i-1} \csrc_i(\tilde v))\comp_i(\ctgt_i(\tilde u) \pcomp_{i-1} \tilde v)
    =
    (\csrc_i(\tilde u) \pcomp_{i-1} \tilde v)\comp_i(\tilde u\pcomp_{i-1} \ctgt_i(\tilde v))
  \end{equation}
  for $(i{-}1)$\composable~$\tilde u,\tilde v \in C_{k}$. If~$i = k-1$, we
  put~$u\comp_i v = u\pcomp_i v$, and the equation~\eqref{eq:parametrized-exch}
  is an instance of~\ref{cond:pcat-to-strict}. Otherwise, if~$i < k-1$, we
  define~$u\comp_i v$ inductively by
  \[
    u\comp_iv=(u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_iv)\zbox.
  \]
  By induction hypothesis, using~\eqref{eq:parametrized-exch}, the above
  definition is equivalent to
  \[
    u\comp_iv= (\csrc_{i+1}(u)\pcomp_iv)\comp_{i+1}(u\pcomp_i\ctgt_{i+1}(v))\zbox.
  \]
  Moreover, if~$i > 0$, then given $(i{-}1)$\composable~$\tilde u,\tilde v \in C_k$, we have
  \begingroup
  \newcommand\uvar{\tilde u\pcomp_{i-1} \csrc_i(\tilde v)}
  \newcommand\uvarp{\tilde u\pcomp_{i-1} \ctgt_i(\tilde v)}
  \newcommand\vvar{\ctgt_i(\tilde u) \pcomp_{i-1} \tilde v}
  \newcommand\vvarp{\csrc_i(\tilde u) \pcomp_{i-1} \tilde v}
  %% règle: long align
  \begin{align*}
    &\phantom{{}={}} (\tilde u\pcomp_{i-1} \csrc_i(\tilde v))\comp_i(\ctgt_i(\tilde u) \pcomp_{i-1} \tilde v) \\
    &= [(\uvar) \pcomp_i \csrc_{i+1}(\vvar)]
      \comp_{i+1} [\ctgt_{i+1}(\uvar) \pcomp_i (\vvar)] \\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
    &= [(\uvar) \pcomp_i (\ctgt_i(\tilde u) \pcomp_{i-1} \csrc_{i+1}(\tilde v))]
      \comp_{i+1} [(\ctgt_{i+1}(\tilde u)\pcomp_{i-1} \csrc_i(\tilde v)) \pcomp_i (\vvar)] \\
    \shortintertextnobreakabove{\hfill(by compatibility of~$\csrctgt\eps_{i+1}$ with~$\pcomp_{i-1}$)}
    &= [(\csrc_i(\tilde u) \pcomp_{i-1} \csrc_{i+1}(\tilde v)) \pcomp_i (\tilde u\pcomp_{i-1} \ctgt_i(\tilde v))]
      \comp_{i+1} [(\csrc_i(\tilde u) \pcomp_{i-1} \tilde v) \pcomp_i (\ctgt_{i+1}(\tilde u)\pcomp_{i-1} \ctgt_i(\tilde v))] \\
    \shortintertextnobreakabove{\hfill(by the condition \ref{cond:pcat-to-strict})}
    &= [\csrc_{i+1}(\csrc_i(\tilde u) \pcomp_{i-1} \tilde v) \pcomp_i (\tilde u\pcomp_{i-1} \ctgt_i(\tilde v))]
      \comp_{i+1} [(\csrc_i(\tilde u) \pcomp_{i-1} \tilde v) \pcomp_i \ctgt_{i+1}(\tilde u\pcomp_{i-1} \ctgt_i(\tilde v))] \\
    \shortintertextnobreakabove{\hfill(by compatibility of~$\csrctgt\eps_{i+1}$ with~$\pcomp_{i-1}$)}
    &=(\csrc_i(\tilde u) \pcomp_{i-1} \tilde v)\comp_i(\tilde u\pcomp_{i-1} \ctgt_i(\tilde v))
      \shortintertextnobreakabove{\hfill(by the equivalent definition of~$\comp_i$)\zbox.}
  \end{align*}
  % on enlève l'espacement dû au strut
  \vskip-\baselineskip\vskip-\jot
  % on passe à un espacement short % en fait pas besoin car on est long en bas
  % \vskip-\belowdisplayskip\vskip\belowdisplayshortskip
  \endgroup \noindent We now prove that the axioms of strict categories are
  satisfied (\cf \myCref[Paragraph~1.4.1.1]{par:ocat-def}).
  \Axr[(i)]{cat:id-srctgt} is a consequence of the precategory
  \Axr{precat:src-tgt-unit}. Given~$i,k \in \N_{n-1}$ with~$i < k$,~$\eps \in
  \set{-,+}$ and $i$\composable~$u,v \in C_{k}$, if~$i = k-1$, then we
  have
  \[
    \csrctgt\eps_{k-1}(u\comp_iv) = \csrctgt\eps_{k-1}(u\pcomp_iv) =
    \begin{cases}
      \csrc_{k-1}(u)& \text{if~$\eps = -$,} \\
      \ctgt_{k-1}(v) & \text{if~$\eps=+$,}
    \end{cases}
  \]
  and otherwise, if~$i < k-1$, we have
  \begin{align*}
    \csrctgt\eps_{k-1}(u\comp_iv) &= \csrctgt\eps_{k-1}((u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_iv))
  \end{align*}
  so that, if~$i +1 = k-1$, when~$\eps = -$ we have
  \[
    \csrctgt\eps_{k-1}(u\comp_iv) =
    \csrc_{k-1}(u\pcomp_i\csrc_{i+1}(v)) = \csrc_{k-1}(u) \pcomp_i
    \csrc_{k-1}(v) = \csrc_{k-1}(u) \comp_i \csrc_{k-1}(v)
  \]
  and similarly~$\csrctgt\eps_{k-1}(u\comp_i v) = \ctgt_{k-1}(u) \comp_i
  \ctgt_{k-1}(v)$ when~$\eps = +$, and finally, if~$i+1 < k-1$, then
  \begin{align*}
    \csrctgt\eps_{k-1}(u\comp_iv)
    &=
      \csrctgt\eps_{k-1}(u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}\csrctgt\eps_{k-1}(\ctgt_{i+1}(u)\pcomp_iv)) \\
    &= (\csrctgt\eps_{k-1}(u)\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_i\csrctgt\eps_{k-1}(v))) \\
    &= \csrctgt\eps_{k-1}(u) \comp_i \csrctgt\eps_{k-1}(v)\zbox.
  \end{align*}
  Thus, \Axr[(ii)]{cat:src-tgt} holds.

  \smallpar We now prove~\Axr[(iii)]{cat:unital}, \ie
  that for~$i,k\in \N_n$ with~$i < k$ and~$u \in C_{k}$, we
  have~$\unitp{k}{\csrc_i(u)} \comp_i u= u$, by induction on~$k - i$ (the dual
  property can be shown similarly). If~$i = k-1$, then the equality is a
  consequence of the unitality of~$\pcomp_i$, by the precategory
  \Axr[(iii)]{precat:compat-id-comp}. Otherwise, if~$i < k-1$, we have
  \begin{align*}
    \unitp{k}{\csrc_i(u)} \comp_i u
    &= (\unitp{k}{\csrc_i(u)} \pcomp_i\csrc_{i+1}(u))
      \comp_{i+1} (\unitp{i+1}{\csrc_i(u)}\pcomp_i u) & \text{(by definition of~$\comp_i$)}\\
    &= \unitp{k}{}(\unitp {i+1}{\csrc_i(u)}\pcomp_i\csrc_{i+1}(u))
      \comp_{i+1} u & \text{(by~\Axr[(iii)]{precat:compat-id-comp})}\\
    &= \unitp{k}{\csrc_{i+1}(u)} \comp_{i+1} u & \text{(by~\Axr[(iii)]{precat:compat-id-comp})}\\
    &= u & \text{(by induction hypothesis)}
  \end{align*}
  so that \Axr[(iii)]{cat:unital} holds.

  \smallpar In order to show \Axr[(iv)]{cat:assoc}, we first prove a
  distributivity property of~$\pcomp_{(-)}$ over~$\comp_{(-)}$, \ie that
  for~$i,j,k \in \N_n$ with~$i < j < k$, given $j$\composable~$u,v \in C_{k}$,
  and~$w \in C_{i+1}$ such that~$u,w$ are $i$\composable, then
  \begin{equation}
    \label{eq:pcat2cat-pcomp-comp-distrib}
    (u\comp_j v)\pcomp_i w = (u\pcomp_i w)\comp_j (v\pcomp_i w).
  \end{equation}
  We prove this property by induction on~$k-j$.
  If~$j = k - 1$, then
  \begin{align*}
    (u\comp_j v)\pcomp_i w &= (u\pcomp_j v)\pcomp_i w \\
                           &=(u\pcomp_i w)\pcomp_j (v\pcomp_i w) & \text{(by \Axr{precat:distrib})}\\
                           &=(u\pcomp_i w)\comp_j (v\pcomp_i w)\pbox.
  \end{align*}
  Otherwise, if~$j < k - 1$, then
  \begin{align*}
    (u\comp_j v)\pcomp_i w
    &= \left[  (u\pcomp_j \csrc_{j+1}(v))\comp_{j+1}(\ctgt_{j+1}(u)\pcomp_j v)\right]\pcomp_i w \\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_j$)}
    &= \left[  (u\pcomp_j \csrc_{j+1}(v))\pcomp_i w\right]\comp_{j+1}\left[  (\ctgt_{j+1}(u)\pcomp_j v)\pcomp_i w \right] \\
    \shortintertextnobreakabove{\hfill(by the induction hypothesis)}
    &= \left[  (u\pcomp_i w)\pcomp_j (\csrc_{j+1}(v)\pcomp_i w)\right]\comp_{j+1}\left[  (\ctgt_{j+1}(u)\pcomp_i w)\pcomp_j (v\pcomp_i w) \right] \\
    \shortintertextnobreakabove{\hfill(by distributivity of~$\pcomp_i$ over~$\pcomp_{j}$)}
    \noalign{\goodbreak}
    &= (u\pcomp_i w)\comp_j (v\pcomp_i w)
      % \shortintertextnobreakabove{\hfill(by definition of~$\comp_j$)\zbox.}
      \shortintertextnobreakabove{\hfill(by \eqref{eq:pcat2cat-pcomp-comp-distrib})\zbox.}
  \end{align*}
  % on enlève l'espacement dû au strut
  \vskip-\baselineskip\vskip-\jot
  % on passe à un espacement short
  \vskip-\belowdisplayskip\vskip\belowdisplayshortskip
  \noindent
  We can now show that~$(u\comp_i v)\comp_i w = u\comp_i (v\comp_i w)$ for
  $i$\composable~$u,v,w\in C_{k}$, for some~$i,k \in \N_n$ with~$i < k$, by
  induction on~$k-i$. If~$i = k-1$, then~$(u\comp_i v)\comp_i w = u\comp_i
  (v\comp_i w)$ by \Axr{precat:assoc}. Otherwise, if~$i < k-1$, we have
  %% règle: long align
  \begin{align*}
    (u\comp_i v)\comp_i w &= \left[ (u\pcomp_i \csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_i v)\right]\comp_i w\\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
                        &= \left\{   \left[ (u\pcomp_i \csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_i v)\right]\pcomp_i \csrc_{i+1}(w) \right\} \\
                        &\phantom{={}}\comp_{i+1} 
                          \left[   (\ctgt_{i+1}(u)\pcomp_i \csrc_{i+1}(v))\pcomp_i w \right]\\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
                        &= \left[ (u\pcomp_i \csrc_{i+1}(v)\pcomp_i \csrc_{i+1}(w))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_i v\pcomp_i \csrc_{i+1}(w))\right] \\
                        &\phantom{={}}\comp_{i+1} 
                          (\ctgt_{i+1}(u)\pcomp_i \csrc_{i+1}(v)\pcomp_i w)\\
    % \shortintertext{\hfill(by distributivity of~$\pcomp_i$ over~$\comp_{i+1}$)}
    \shortintertextnobreakabove{\hfill(by \eqref{eq:pcat2cat-pcomp-comp-distrib})}
                        &=  (u\pcomp_i \csrc_{i+1}(v)\pcomp_i \csrc_{i+1}(w)) \\*
                        &\phantom{={}}\comp_{i+1}\left[ (\ctgt_{i+1}(u)\pcomp_i v\pcomp_i \csrc_{i+1}(w))
                          \comp_{i+1} 
                          (\ctgt_{i+1}(u)\pcomp_i \csrc_{i+1}(v)\pcomp_i w )\right]\\*
    \shortintertextnobreakabove{\hfill(by associativity of~$\comp_{i+1}$ from induction hypothesis)}
                        &=  \left[  u\pcomp_i (\csrc_{i+1}(v)\pcomp_i \csrc_{i+1}(w)) \right]\\*
                        &\phantom{={}}\comp_{i+1}\left\{ \ctgt_{i+1}(u)\pcomp_i \left[  (v\pcomp_i \csrc_{i+1}(w))
                          \comp_{i+1} 
                          (\csrc_{i+1}(v)\pcomp_i w )\right]\right\}\\
    % \shortintertext{\hfill(by distributivity of~$\pcomp_i$ over~$\comp_{i+1}$)}
    \shortintertextnobreakabove{\hfill(by \eqref{eq:pcat2cat-pcomp-comp-distrib})}
    \noalign{\goodbreak}
                        &= u\comp_i \left[ (v\pcomp_i \csrc_{i+1}(w))
                          \comp_{i+1} 
                          (\csrc_{i+1}(v)\pcomp_i w ) \right] \\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
                        &=u\comp_i (v\comp_i w)\\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
  \end{align*}
  % la proposition d'espacement suivante semble fonctionner
  % on enlève l'espacement dû au strut
  \vskip-\baselineskip\vskip-\jot
  % on passe à un espacement short
  \vskip-\belowdisplayskip\vskip\belowdisplayshortskip
  % 
  \noindent which concludes the proof of \Axr{cat:assoc}.

  \smallpar We now prove~\ref{cat:id-xch}, \ie that for~$i,k \in \N_{n-1}$
  with~$i < k$, and $i$\composable~$u,v\in C_{k}$, we
  have~$\unitp{k+1}{u}\comp_i\unitp{k+1}{v} = \unitp{k+1}{u\comp_iv}$, by
  induction on~$k-i$. If~$i = k-1$, then
  \begin{align*}
    \unitp{k+1}{u}\comp_i \unitp{k+1}{v}
    &= (\unitp{k+1}{u}\pcomp_i v)\comp_{i+1}(u\pcomp_i \unitp{k+1}{v}) & \text{(by definition of~$\comp_i$)}\\
    &= \unitp{k+1}{u\pcomp_i v}\pcomp_{i+1}\unitp{k+1}{u\pcomp_i v} &\text{(by~\ref{precat:compat-id-comp})}\\
    &= \unitp{k+1}{u\pcomp_i v} &\text{(by~\ref{precat:compat-id-comp})\zbox.}
  \end{align*}
  Otherwise, if~$i < k-1$, then
  \begin{align*}
    \unitp{k+1}{u}\comp_i\unitp{k+1}{v}
    &=(\unitp{k+1}{u}\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_i\unitp{k+1}{v}) & \text{(by definition of~$\comp_i$)}\\
    &=\unitp{k+1}{}(u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}\unitp{k+1}{}(\ctgt_{i+1}(u)\pcomp_iv) & \text{(by~\ref{precat:compat-id-comp})} \\
    &=\unitp{k+1}{}((u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_iv)) & \text{(by induction hypothesis)}\\
    &=\unitp{k+1}{u\comp_iv} & \text{(by definition of~$\comp_i$)}
  \end{align*}
  so that \Axr{cat:id-xch} holds.

  \smallpar Finally, we show \Axr{cat:xch}, \ie that for~$i,j,k \in \N_n$
  with~$i < j < k$, $j$\composable~$u,u'\in C_{k}$ and
  $j$\composable~$v,v'\in C_{k}$ such that~$u,v$ are $i$\composable, we have
  \[
    (u\comp_ju')\comp_i(v\comp_jv')=(u\comp_iv)\comp_j(u'\comp_iv')
  \]
  by induction on~$j-i$. If~$i = j-1$, then we have
  \begingroup
  \allowdisplaybreaks
  \begin{align*}
    (u\comp_ju')\comp_i(v\comp_jv')
    &=
      \left[ (u\comp_{i+1}u')\pcomp_i\csrc_{i+1}(v) \right] \comp_{i+1} \left[ \ctgt_{i+1}(u')\pcomp_i(v\comp_{i+1}v') \right] \\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
    &=
      (u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(u'\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u')\pcomp_iv)\comp_{i+1}(\ctgt_{i+1}(u')\pcomp_iv') \\
    % \shortintertext{\hfill(by the distributivity property of~$\pcomp_i$ over~$\comp_{i+1}$)}
    \shortintertextnobreakabove{\hfill(by \eqref{eq:pcat2cat-pcomp-comp-distrib})}
    &=
      (u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\csrc_{i+1}(u')\pcomp_iv)\comp_{i+1}(u'\pcomp_i\ctgt_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u')\pcomp_iv') \\
    \shortintertextnobreakabove{\hfill(by \eqref{eq:parametrized-exch})}
    &= (u\comp_iv)\comp_j(u'\comp_iv')
      \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)\zbox.}
  \end{align*}
  \endgroup
  % on enlève l'espacement dû au strut
  \vskip-\baselineskip\vskip-\jot
  % on passe à un espacement short
  \vskip-\belowdisplayskip\vskip\belowdisplayshortskip
  \noindent Otherwise, if~$i < j-1$, then we have
  \begingroup
  \allowdisplaybreaks
  \begin{align*}
    (u\comp_ju')\comp_i(v\comp_jv')
    &=
      \left[ (u\comp_ju')\pcomp_i\csrc_{i+1}(v) \right]\comp_{i+1}\left[ \ctgt_{i+1}(u')\pcomp_i(v\comp_jv') \right]\\
    \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
    &=
      \left[ (u\pcomp_i\csrc_{i+1}(v))\comp_j(u'\pcomp_i\csrc_{i+1}(v)) \right]\comp_{i+1}\left[ (\ctgt_{i+1}(u')\pcomp_iv)\comp_j(\ctgt_{i+1}(u')\pcomp_iv') \right]\\
    %\shortintertext{\hfill(by the distributivity property of~$\pcomp_i$ over~$\comp_{i+1}$)}
    \shortintertextnobreakabove{\hfill(by \eqref{eq:pcat2cat-pcomp-comp-distrib})}
    &=
      \left[ (u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u')\pcomp_iv) \right]\comp_{j}\left[ (u'\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u')\pcomp_iv') \right]\\
    \shortintertextnobreakabove{\hfill(by the induction hypothesis)}
    &=
      \left[ (u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_iv) \right]\comp_{j}\left[ (u'\pcomp_i\csrc_{i+1}(v'))\comp_{i+1}(\ctgt_{i+1}(u')\pcomp_iv') \right]\\
    \shortintertextnobreakabove{\hfill(by~$j$-composability of~$u,u'$ and~$v,v'$ and the globular structure)}
    \noalign{\goodbreak}
    &=
      (u\comp_iv)\comp_j(u'\comp_iv')
      \shortintertextnobreakabove{\hfill(by definition of~$\comp_i$)}
  \end{align*}
  \endgroup
  % on enlève l'espacement dû au strut
  \vskip-\baselineskip\vskip-\jot
  % on passe à un espacement short
  \vskip-\belowdisplayskip\vskip\belowdisplayshortskip
  \noindent which concludes the proof of \Axr{cat:xch}. Hence,~$C$ is equipped
  with a structure of strict $n$\category.

  Thus, for~$n \in \Ninf$, we have defined a mapping~$\bar\Theta^n$ between the
  objects of~$\nPCatstr n$ and the objects of~$\nCat n$. We show
  that~$\bar\Theta^n$ extends to a functor~$\bar\Theta^n \co \nPCatstr n \to
  \nCat n$. Given an $n$\prefunctor~$F \co C \to C'$ between two
  $n$\precategories~$C$ and~$C'$ which satisfy~\ref{cond:pcat-to-strict}, it is
  sufficient to show that~$F$ is compatible with the~$\comp_{(-)}$ operations.
  Given~$i,k \in \N_n$ with~$i < k$, and~$u,v \in C_{k}$ such that~$u,v$ are
  $i$\composable, we prove that~$F(u\comp_iv) = F(u) \comp_i F(v)$ by induction
  on~$k - i$. If~$i = k-1$, we have
  \[
    F(u\comp_iv) = F(u\pcomp_i v) = F(u)\pcomp_i F(v) = F(u)\comp_iF(v)\zbox.
  \]
  Otherwise, if~$i < k-1$, we have
  \begin{align*}
    F(u\comp_iv) &= F((u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_iv)) \\
                 &= (F(u)\pcomp_iF(\csrc_{i+1}(v)))\comp_{i+1}(F(\ctgt_{i+1}(u))F(\pcomp_iv)) & \text{(by induction hypothesis)} \\
                 &= F(u)\comp_iF(v)
  \end{align*}
  which concludes the proof that~$F$ induces an $n$\functor.
\end{proof}

\paragraph{Equivalence of the definitions}

In this section, we conclude that, for~$n \in \Ninf$, $n$\categories can be
equivalently described as $n$\precategories
satisfying~\ref{cond:pcat-to-strict}. More precisely, we show~$\Theta^n$
and~$\bar\Theta^n$ witness that~$\nCat n$ and~$\nPCatstr n$ isomorphic to each
other. We first show that:
\begin{prop}
  Given~$n \in \Ninf$ and~$C \in \nCat n$, we have~$\bar\Theta^n\Theta^n C = C$.
\end{prop}
\begin{proof}
  Let~$\comp_{(-)}$ be the composition operations of~$C$,~$\pcomp_{(-)}$ be the
  composition operations of~$\Theta^n C$, and~$\comp'_{(-)}$ be the composition
  operations of~$\bar\Theta^n\Theta^n C$. Given~$i,k \in \N$ with~$i < k \le n$,
  and~$u,v \in C_{k}$ such that~$u,v$ are $i$\composable, we prove
  that~$u\comp'_iv = u \comp_i v$ by induction on~$k - i$. If~$i = k-1$, we have
  \[
    u\comp'_iv = u\pcomp_iv = u\comp_iv\zbox.
  \]
  Otherwise, if~$i < k-1$, we have
  \begin{align*}
    u\comp'_iv &= (u\pcomp_i\csrc_{i+1}(v)\comp'_{i+1}(\ctgt_{i+1}(u)\pcomp_iv)) \\
                 &= (u\pcomp_i\csrc_{i+1}(v))\comp_{i+1}(\ctgt_{i+1}(u)\pcomp_iv) & \text{(by induction hypothesis)} \\
                 &= (u\comp_i\unitp k {} (\csrc_{i+1}(v)))\comp_{i+1}(\unitp k {}(\ctgt_{i+1}(u))\comp_iv) \\
                 &= (u\comp_{i+1}\unitp k {}(\ctgt_{i+1}(u)))\comp_{i}(\unitp k {} (\csrc_{i+1}(v))\comp_{i+1}v) & \text{(by \Axr{cat:xch})}\\
                 &= u\comp_iv\zbox.
  \end{align*}
  Hence,~$\comp_{(-)} = \comp'_{(-)}$.
\end{proof}
\noindent We now prove the converse property:
\begin{prop}
  Given~$n \in \Ninf$ and~$C \in \nPCatstr n$, we have~$\Theta^n\bar\Theta^n C = C$.
\end{prop}
\begin{proof}
  Let~$\pcomp_{(-)}$ be the composition operations of~$C$,~$\comp_{(-)}$ be the
  composition operations of~$\bar\Theta^nC$, and~$\pcomp'_{(-)}$ be the
  composition operations of~$\Theta^n\bar\Theta^n C$. We show that~$\pcomp_{(-)}
  = \pcomp'_{(-)}$. Given~$i,k,l \in \N_n$ with~$i = \min(k,l) - 1$
  and~$\max(k,l) \le n$, and~$u \in C_k,v \in C_l$ such that~$u,v$ are
  $i$\composable, we show that~$u \pcomp_i v = u \pcomp'_i v$. We can suppose
  that~$k \le l$ (the case~$k \ge l$ is symmetric). If~$k = l$, then
  \begin{align*}
    u\pcomp'_i v = u \comp_i v = u\pcomp_i v 
  \end{align*}
  Otherwise, if~$k < l$, then
  \begin{align*}
    u\pcomp'_i v &= \unitp l u \comp_i v \\
                 &= (\unitp l u \pcomp_i \csrc_{i+1}(v)) \comp_{i+1} (\ctgt_{i+1}(u) \pcomp_i v) \\
                 &= (\unitp l {} (u \pcomp_i \csrc_{i+1}(v))) \comp_{i+1} (u \pcomp_i v) & \text{(by \Axr{precat:compat-id-comp})}\\
                 &= u\pcomp_i v & \text{(by \Axr{cat:unital})\zbox.}
  \end{align*}
  Hence,~$\pcomp_{(-)} = \pcomp'_{(-)}$.
\end{proof}
\noindent By the two above properties, we can conclude that:
\begin{theo}
  \label{prop:strcat-pcat-isom}
  For~$n \in \Ninf$,~$\Theta^n\co \nCat n \to \nPCatstr n$ is an isomorphism of
  categories, with inverse given by~$\bar\Theta^n$.
\end{theo}
\noindent Thus, for~$n \in \Ninf$, a strict $n$\category~$C$ is canonically an
$n$\precategory satisfying~\ref{cond:pcat-to-strict} (and \viceversa). In the
following, we will often use the precategorical compositions~$\pcomp_{(-)}$
of~$C$ without invoking \Cref{prop:strcat-pcat-isom}.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "proxy-strcat-precat"
%%% TeX-command-extra-options: "-shell-escape"
%%% End:
